Investigation of Rocket Effect in BRC 18 using Gaia EDR3

Bright-rimmed clouds (BRCs) are ideal candidates to study radiation-driven implosion mode of star formation as they are potential sites of triggered star formation, located at the edges of H{\sc ii} regions, showing evidence of ongoing star formation processes. BRC 18 is located towards the eastern edge of relatively closer ($\sim$400 pc) H{\sc ii} region excited by $\lambda$ Ori. We made R-band polarimetric observations of 17 candidate young stellar objects (YSOs) located towards BRC 18 to investigate any preferred orientation of the discs with respect to the ambient magnetic field and the direction of energetic photons from $\lambda$ Ori. We found that the discs are oriented randomly with respect to the projected magnetic field. Using distances and proper motions from the \textit{Gaia} EDR3 of the candidate YSOs, we investigated the possible acceleration of BRC 18, away from $\lambda$ Ori due to the well known "Rocket Effect", by assuming that both the candidate YSOs and BRC 18 are kinematically coupled. The relative proper motions of the candidate YSOs are found to show a trend of moving away from $\lambda$ Ori. We computed the offset between the angle of the direction of the ionization front and the relative proper motion of the candidate YSOs and found it to lie close to being parallel to each other. Additionally, we found 12 sources that are comoving with the known candidate YSOs towards BRC 18. These comoving sources are most likely to be young and are missed in previous surveys conducted to identify potential YSOs of the region.

==> Investigation of Rocket Effect in BRC 18_accepted_final_final_arxiv/table_comoving1.tex <==
\begin{table*}
    \begin{center}
    \caption{Properties of the newly found comoving sources identified towards BRC 18 from \textit{Gaia} EDR3.}
    \label{tab:comoving_gaia}
    \renewcommand{\arraystretch}{1.3}
    \scriptsize
    \begin{tabular}{lccccccccccc} 
    \hline
    \#& Source ID& RA(2016)  & Dec(2016)  & $\Delta$RA& $\Delta$Dec&$d\pm\Delta d$ & $\mu_{\alpha\star}\pm\Delta\mu_{\alpha\star}$ & $\mu_{\delta}\pm\Delta\mu_{\delta}$ & $G\pm\Delta G$ & $G_\mathrm{BP}\pm\Delta G_\mathrm{BP}$ & $G_\mathrm{RP}\pm\Delta G_\mathrm{RP}$\\
     & (\textit{Gaia} EDR3) & ($^{\circ}$) & ($^{\circ}$) & ($^{\prime\prime}$) & ($^{\prime\prime}$) &(pc)& (mas yr$^{-1}$) & (mas yr$^{-1}$) & (mag)&(mag)&(mag)\\
     (1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)&(11)&(12)\\
    \hline
1  & 3336166837021667584 & 85.679980 & 9.228623 & 6728.5 &-2539.9 &407$_{-27}^{21}$ & 1.911$\pm$0.161 & -2.499$\pm$0.108 & 17.851$\pm$0.003 & 20.035$\pm$0.072 & 16.481$\pm$0.006\\
2  & 3336149455287469824 & 85.846633 & 9.091804 & 7321.6 &-3032.4 &405$_{-14}^{20}$ & 2.568$\pm$0.113 & -2.309$\pm$0.079 & 16.151$\pm$0.003&-&-\\
3  & 3336156048063746304 & 85.940706 & 9.171731 & 7654.7 &-2744.7 &400$_{-17}^{29}$ & 2.128$\pm$0.123 & -2.704$\pm$0.085 & 17.312$\pm$0.003 & 19.461$\pm$0.034 & 15.921$\pm$0.005\\
4  & 3336111071166289152 & 86.069824 & 9.222508 & 8112.5 &-2561.9 &371$_{-12}^{11}$ & 2.510$\pm$0.098 & -2.494$\pm$0.064 & 17.234$\pm$0.004 & 18.898$\pm$0.046 & 15.751$\pm$0.006\\    
5  & 3336104134795404928 & 86.093515 & 9.044528 & 8198.7 &-3202.6 &401$_{-19}^{19}$ & 2.066$\pm$0.143 & -2.546$\pm$0.088 & 17.408$\pm$0.003 & 19.350$\pm$0.034 & 16.072$\pm$0.005\\
6  & 3336108391106615168 & 86.102807 & 9.163186 & 8230.3 &-2775.5 &403$_{-27}^{19}$ & 2.356$\pm$0.147 & -2.626$\pm$0.093 & 17.930$\pm$0.003 & 19.966$\pm$0.042 & 16.601$\pm$0.007\\
7  & 3336252564567949824 & 86.151543 & 9.308982 & 8401.5 &-2250.6 &389$_{-21}^{25}$ & 2.636$\pm$0.163 & -2.223$\pm$0.106 & 18.262$\pm$0.003 & 20.685$\pm$0.083 & 16.846$\pm$0.007\\
8  & 3336205663525068800 & 86.181870 & 9.299059 & 8509.3 &-2286.3 &385$_{-22}^{27}$ & 3.195$\pm$0.199 & -2.558$\pm$0.132 &  18.311$\pm$0.003 & 20.480$\pm$0.070 & 16.893$\pm$0.007\\
9  & 3336110182109326208 & 86.182331 & 9.192329 & 8512.2 &-2670.6 &386$_{-17}^{15}$ & 2.511$\pm$0.135 & -2.360$\pm$0.080 & 17.502$\pm$0.003 & 19.949$\pm$0.048 & 16.067$\pm$0.005\\
10 & 3336107364610774272 & 86.219055 & 9.209368 & 8642.4 &-2609.2 &375$_{-8}^{8}$ & 3.337$\pm$0.070 & -2.662$\pm$0.045 & 16.628$\pm$0.003 & 18.785$\pm$0.018 & 15.263$\pm$0.005\\
11 & 3336092830441451008 & 86.330422 & 9.056243 & 9039.8 &-3160.5 &389$_{-15}^{23}$ & 2.802$\pm$0.145 & -2.712$\pm$0.076 &  17.316$\pm$0.003 & 19.503$\pm$0.031 & 15.971$\pm$0.005\\
12 & 3336092864798790144 & 86.343198 & 9.070070 & 9084.9 &-3110.7 &402$_{-4}^{3}$ & 2.441$\pm$0.020 & -2.507$\pm$0.012 & 9.266$\pm$0.003 & 10.029$\pm$0.004 & 8.360$\pm$0.005\\
    \hline
    \end{tabular}\\
    \end{center}
\end{table*}

==> Investigation of Rocket Effect in BRC 18_accepted_final_final_arxiv/table_log.tex <==
\begin{table}
	\centering
	\caption{Log of R-band polarimetric observations in the year of 2016.}
	\label{tab:log_obs_brc18}
	\begin{tabular}{lc}
		\hline
		Month (Date) & Heliocentric Julian Date\\\hline%\hline
        October 26 & 2457688.2964\\
        October 28 & 2457690.2963\\
        November 22 & 2457715.2945\\
        November 23 & 2457716.2944\\
        November 24 & 2457717.2943\\
        November 25 & 2457718.2942\\ 
        November 26 & 2457719.2941\\
        November 27 & 2457720.2940\\
        \hline    
	\end{tabular}\\
\end{table}

==> Investigation of Rocket Effect in BRC 18_accepted_final_final_arxiv/table_yso1.tex <==
\begin{table*}
	\begin{center}
		\caption{Properties of the previously known candidate YSOs towards BRC 18 from \textit{Gaia} EDR3.}
		\label{tab:yso_gaia}
		\renewcommand{\arraystretch}{1.3}
		\scriptsize
		\begin{tabular}{lccccccccccc} 
			\hline
			\#& Source ID& RA(2016)  & Dec(2016)  & $\Delta$RA & $\Delta$Dec & $d\pm\Delta d$ & $\mu_{\alpha\star}\pm\Delta\mu_{\alpha\star}$ & $\mu_{\delta}\pm\Delta\mu_{\delta}$ & $G\pm\Delta G$ & $G_\mathrm{BP}\pm\Delta G_\mathrm{BP}$ & $G_\mathrm{RP}\pm\Delta G_\mathrm{RP}$\\
			& (\textit{Gaia} EDR3) & ($^{\circ}$) & ($^{\circ}$) & ($^{\prime\prime}$) & ($^{\prime\prime}$) & (pc)& (mas yr$^{-1}$) & (mas yr$^{-1}$) & (mag)&(mag)&(mag)\\
			(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)&(11)&(12)\\
			\hline
1  & 3336168314489240704 & 85.660435 & 9.310332 & 6658.4 &-2245.7&397$_{-4}^{4}$& 2.054$\pm$0.026 & -2.187$\pm$0.018 & 14.580$\pm$0.003 & 15.405$\pm$0.009 & 13.665$\pm$0.007\\
2  & 3336168043908536704 & 85.680581 & 9.287969 & 6730.1 &-2326.3&383$_{-9}^{8}$& 1.409$\pm$0.070 & -2.557$\pm$0.047 & 16.419$\pm$0.003 & 18.436$\pm$0.018 & 15.080$\pm$0.005\\
3  & 3336155189070384384 & 85.729819 & 9.246989 & 6905.3 &-2473.8&390$_{-6}^{6}$& 2.076$\pm$0.054 & -2.141$\pm$0.037 & 15.995$\pm$0.003 & 17.431$\pm$0.008 & 14.818$\pm$0.005\\		
4  & 3336152375867856512 & 85.747103 & 9.164555 & 6967.5 &-2770.5&390$_{-4}^{6}$& 1.506$\pm$0.035 & -2.735$\pm$0.025 & 15.059$\pm$0.003 & 16.172$\pm$0.012 & 13.977$\pm$0.005\\			
5  & 3336161549917961088 & 85.802402 & 9.283812 & 7162.5 &-2341.2&394$_{-4}^{5}$& 2.011$\pm$0.036 & -2.482$\pm$0.023 & 15.179$\pm$0.005 & 16.392$\pm$0.020 & 14.070$\pm$0.012\\	
6  & 3336180585212965376 & 85.814037 & 9.491866 & 7201.6 &-1592.2&407$_{-4}^{5}$ & 2.137$\pm$0.027 & -2.488$\pm$0.018 & 14.675$\pm$0.003 & 15.555$\pm$0.021 & 13.638$\pm$0.008\\
7  & 3336160690924950272 & 85.873411 & 9.283380 & 7414.6 &-2342.8&400$_{-9}^{10}$& 2.180$\pm$0.077 & -2.473$\pm$0.046 & 16.390$\pm$0.003 & 17.857$\pm$0.015 & 15.201$\pm$0.005\\
8  & 3336177454181082496 & 85.890385 & 9.496435 & 7472.5 &-1575.8&401$_{-15}^{13}$& 2.106$\pm$0.091 & -2.722$\pm$0.065 & 17.316$\pm$0.003 & 19.431$\pm$0.025 & 15.958$\pm$0.005\\
9  & 3336156121079561344 & 85.914989 & 9.178026 & 7563.3 &-2722.0&370$_{-9}^{15}$& 2.170$\pm$0.103 & -2.299$\pm$0.065 & 16.676$\pm$0.003 & 18.491$\pm$0.017 & 15.345$\pm$0.005\\
10 & 3336149867606924288 & 85.935460 & 9.133633 & 7636.5 &-2881.9&429$_{-32}^{30}$ & 1.069$\pm$0.183 & -2.405$\pm$0.116 & 18.321$\pm$0.010 & 19.229$\pm$0.048 & 17.202$\pm$0.031\\
11 & 3336156292877976064 & 85.961132 & 9.206919 & 7726.8 &-2618.0&405$_{-9}^{11}$& 2.422$\pm$0.065 & -2.415$\pm$0.040 & 16.295$\pm$0.010 & 17.859$\pm$0.040 & 15.057$\pm$0.024\\
12 & 3336157422453353600 & 85.963992 & 9.227901 & 7736.7 &-2542.5&399$_{-31}^{30}$& 2.189$\pm$0.219 & -2.004$\pm$0.145 & 18.391$\pm$0.003 & 20.377$\pm$0.074 & 16.975$\pm$0.010\\
13 & 3336159419614147584 & 85.968111 & 9.283435 & 7750.7 &-2342.6&394$_{-7}^{6}$& 2.690$\pm$0.046 & -2.470$\pm$0.031 & 15.716$\pm$0.003 & 17.415$\pm$0.006 & 14.464$\pm$0.004\\
14 & 3336157873425924992 & 85.968650 & 9.266585 & 7752.8 &-2403.2&384$_{-15}^{13}$& 2.227$\pm$0.107 & -2.585$\pm$0.074 & 17.422$\pm$0.003 & 19.441$\pm$0.035 & 16.078$\pm$0.006\\
15 & 3336102897844569856 & 85.972911 & 9.119901 & 7769.6 &-2931.3&394$_{-9}^{8}$& 1.414$\pm$0.066 & -2.423$\pm$0.043 & 16.228$\pm$0.009 & 17.575$\pm$0.043 & 15.000$\pm$0.025\\	
16 & 3336159557053093248 & 85.985790 & 9.304671 & 7813.2 &-2266.1&371$_{-9}^{9}$& 2.388$\pm$0.062 & -2.181$\pm$0.044 & 16.397$\pm$0.016 & 17.831$\pm$0.051 & 15.204$\pm$0.043\\
17 & 3336159282175185792 & 86.006802 & 9.289093 & 7888.0 &-2322.2&393$_{-4}^{5}$& 2.753$\pm$0.028 & -2.600$\pm$0.019 & 14.750$\pm$0.003 & 15.793$\pm$0.008 & 13.726$\pm$0.005\\		
18 & 3336109048235617536 & 86.041829 & 9.144624 & 8014.0 &-2842.3&414$_{-13}^{12}$& 1.884$\pm$0.090 & -2.221$\pm$0.052 & 16.814$\pm$0.008 & 17.926$\pm$0.035 & 15.703$\pm$0.015\\
19 & 3336107429033839360 & 86.053240 & 9.086216 & 8055.2 &-3052.6&391$_{-8}^{9}$& 1.496$\pm$0.075 & -2.510$\pm$0.046 & 16.625$\pm$0.004 & 18.211$\pm$0.013 & 15.350$\pm$0.014\\			
20 & 3336108223604259456 & 86.061986 & 9.135564 & 8085.7 &-2874.9&385$_{-8}^{7}$& 1.588$\pm$0.050 & -2.323$\pm$0.031 & 15.728$\pm$0.003 & 17.242$\pm$0.009 & 14.524$\pm$0.007\\
21 & 3336111006743055360 & 86.079400 & 9.209260 & 8146.6 &-2609.6&382$_{-12}^{7}$ & 2.229$\pm$0.078 & -2.416$\pm$0.048 & 16.458$\pm$0.003 & 18.186$\pm$0.023 & 15.024$\pm$0.005\\
22 & 3336158594980405376 & 86.080847 & 9.271995 & 8151.0 &-2383.8&409$_{-9}^{12}$& 1.613$\pm$0.056 & -2.534$\pm$0.036 & 16.170$\pm$0.003 & 17.742$\pm$0.009 & 14.948$\pm$0.005\\
23 & 3336158521965029760 & 86.087587 & 9.267106 & 8175.0 &-2401.4&382$_{-7}^{8}$& 2.546$\pm$0.061 & -2.198$\pm$0.039 & 16.189$\pm$0.003 & 17.999$\pm$0.009 & 14.910$\pm$0.004\\			
24 & 3336108361043207040 & 86.090606 & 9.148215 & 8187.2 &-2829.4&399$_{-8}^{9}$& 1.699$\pm$0.061 & -2.753$\pm$0.039 & 15.938$\pm$0.003 & 17.824$\pm$0.022 & 14.462$\pm$0.007\\
25 & 3336109937294863744 & 86.095395 & 9.176425 & 8203.8 &-2727.8&394$_{-5}^{6}$& 2.635$\pm$0.035 & -2.412$\pm$0.022 & 15.059$\pm$0.003 & 16.228$\pm$0.006 & 13.978$\pm$0.005\\
26 & 3336110834944361984 & 86.107235 & 9.200320 & 8245.6 &-2641.8&387$_{-8}^{7}$& 3.095$\pm$0.057 & -2.596$\pm$0.036 & 16.160$\pm$0.003 & 17.781$\pm$0.015 & 14.913$\pm$0.007\\
27 & 3336109902935129088 & 86.112112 & 9.178385 & 8263.1 &-2720.8&393$_{-6}^{8}$ & 2.891$\pm$0.056 & -2.444$\pm$0.035 & 16.221$\pm$0.003 & 17.718$\pm$0.007 & 15.033$\pm$0.004\\
28 & 3336104955132704640 & 86.119424 & 9.105122 & 8290.0 &-2984.5&416$_{-22}^{27}$& 2.933$\pm$0.150 & -2.390$\pm$0.097 & 17.918$\pm$0.003 & 20.044$\pm$0.062 & 16.563$\pm$0.007\\
29 & 3336256176637551232 & 86.137795 & 9.446547 & 8351.0 &-1755.4&383$_{-4}^{3}$& 2.782$\pm$0.029 & -1.843$\pm$0.019 & 14.865$\pm$0.003 & 16.315$\pm$0.004 & 13.683$\pm$0.004\\
30 & 3336110525706709120 & 86.154261 & 9.222194 & 8412.2 &-2563.0&384$_{-6}^{7}$& 2.709$\pm$0.043 & -2.393$\pm$0.027 & 15.580$\pm$0.003 & 17.301$\pm$0.008 & 14.309$\pm$0.005\\
31 & 3336104787630415616 & 86.157234 & 9.099283 & 8424.3 &-3005.5&409$_{-9}^{11}$& 2.625$\pm$0.081 & -2.558$\pm$0.053 & 16.663$\pm$0.003 & 18.792$\pm$0.018 & 15.309$\pm$0.004\\
32 & 3336256103621173504 & 86.158848 & 9.432716 & 8425.9 &-1805.2&420$_{-13}^{16}$& 1.832$\pm$0.081 & -2.203$\pm$0.056 & 17.188$\pm$0.003 & 18.984$\pm$0.027 & 15.912$\pm$0.005\\
33 & 3336107227171825664 & 86.194115 & 9.189299 & 8554.1 &-2681.5&402$_{-6}^{6}$& 3.053$\pm$0.041 & -2.504$\pm$0.027 & 15.667$\pm$0.003 & 16.959$\pm$0.008 & 14.528$\pm$0.005\\
34 & 3335326299037613056 & 86.226617 & 8.713875 & 8675.5 &-4393.0&417$_{-13}^{14}$& 2.009$\pm$0.088 & -2.621$\pm$0.059 & 17.223$\pm$0.017 & 19.321$\pm$0.081 & 15.809$\pm$0.046\\
    \hline
\end{tabular}\\
\end{center}
\end{table*}

==> Investigation of Rocket Effect in BRC 18_accepted_final_final_arxiv/table_yso_pol_new5.tex <==
\begin{table}
    \scriptsize
		\centering
		\caption{Results of R-band polarization measurements of the observed candidate YSOs towards BRC 18 along with the astrometric and photometric properties obtained from \textit{Gaia} EDR3.}
		%\subcaption*{Sources having reliable counterparts in \textit{Gaia} EDR3}
		\label{tab:sources_p_pa_new}
		\renewcommand{\arraystretch}{1.5}
		\begin{tabular}{ccccccccccccccc}			
			\hline
			Serial & Source ID & RA$^{*}$ & Dec$^{*}$ & $\Delta$RA$^{\dagger}$ & $\Delta$Dec$^{\dagger}$ & P$\pm\Delta$P & $\theta$$\pm$$\Delta\theta$ & $d$$\pm$$\Delta d$ & $\mu_{\alpha\star}$$\pm$$\Delta\mu_{\alpha\star}$ & $\mu_{\delta}$$\pm\Delta$$\mu_{\delta}$ & RUWE & $G$$\pm\Delta$$G$$^{\ddagger}$&$G_\mathrm{BP}$$\pm$$\Delta G_\mathrm{BP}$$^{\ddagger}$ & $G_\mathrm{RP}$$\pm$$\Delta G_\mathrm{RP}$$^{\ddagger}$\\
			No.& (\textit{Gaia} EDR3) & ($^{\circ}$) & ($^{\circ}$) & ($^{\prime\prime}$) & ($^{\prime\prime}$) & (\%) & ($^{\circ}$) & (pc) & (mas yr$^{-1}$) & (mas yr$^{-1}$)&&(mag)&(mag)&(mag)\\ 
			(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)&(11)&(12)&(13)&(14)&(15)\\
			\hline
			\multicolumn{15}{c}{Sources having reliable counterparts in \textit{Gaia} EDR3}\\
			1 &3336149519712868736 &85.837176 & 9.101955 & 7287.9 &-2995.9&0.4$\pm$0.2 & 177$\pm$9 & 402$_{-3}^{4}$ & 2.145$\pm$0.021 & -2.665$\pm$0.015 &1.376& 12.581$\pm$0.012&13.343$\pm$0.043 & 11.691$\pm$0.030\\
			2 &3336159071720837120 &86.008674 &9.260364 & 7895.0 &-2425.6&2.3$\pm$0.3& 95$\pm$3 & 387$_{-5}^{5}$& 2.257$\pm$0.031 & -2.482$\pm$0.022 &1.012& 15.074$\pm$0.004&16.394$\pm$0.014 & 13.931$\pm$0.008\\	
			3 &3336107772631258624 &86.030253 & 9.110574 & 7973.3 &-2964.9&0.6$\pm$0.2 & 176$\pm$7 &393$_{-3}^{4}$ &1.661$\pm$0.031 &-2.703$\pm$0.018 &1.381& 13.694$\pm$0.004&14.458$\pm$0.012& 12.794$\pm$0.008\\
			4 &3336109563633776896 &86.044381 & 9.212530 & 8022.3 &-2597.8&0.7$\pm$0.2 & 182$\pm$10 & 396$_{-3}^{3}$ & 2.595$\pm$0.019 & -2.488$\pm$0.012 &1.094& 13.798$\pm$0.003&14.499$\pm$0.004& 12.985$\pm$0.004\\
			5 &3336104581471997440 &86.080668 & 9.089784 & 8152.6 &-3039.7&0.7$\pm$0.4& 147$\pm$11& 383$_{-5}^{5}$& 2.702$\pm$0.044 & -2.640$\pm$0.027 &1.059& 15.461$\pm$0.003&16.818$\pm$0.006& 14.313$\pm$0.004\\
			6 &3336108361043206912 &86.091194 & 9.147915 & 8189.2 &-2830.4&1.6$\pm$0.3 & 67$\pm$6 & 393$_{-3}^{4}$ & 2.250$\pm$0.028 & -2.483$\pm$0.018 &1.122& 14.513$\pm$0.003&15.707$\pm$0.008& 13.389$\pm$0.008\\
			7 &3336105028148587904 &86.108237 & 9.116840 & 8250.1 &-2942.3&0.7$\pm$0.2 & 179$\pm$10 &397$_{-2}^{3}$ & 2.571$\pm$0.018 & -2.720$\pm$0.011 &1.057& 13.645$\pm$0.008&14.488$\pm$0.026& 12.710$\pm$0.023\\	
			8 &3336204155993987200 &86.220057 & 9.218111 & 8645.8 &-2577.7&2.4$\pm$0.2 & 83$\pm$4 & 391$_{-2}^{4}$ & 1.909$\pm$0.022 & -2.321$\pm$0.014 &1.153& 14.141$\pm$0.005&14.968$\pm$0.014& 13.230$\pm$0.013\\
			9 &3336093513339795200 &86.267100 & 9.081243 & 8814.6 &-3070.5&1.0$\pm$0.3 &128$\pm$7 &394$_{-5}^{6}$ &2.323$\pm$0.038 & -2.859$\pm$0.022 &0.960& 15.178$\pm$0.004&16.482$\pm$0.011& 14.040$\pm$0.009\\
			\hline
			\multicolumn{15}{c}{Sources having unreliable counterparts in \textit{Gaia} EDR3}\\
			10 &3336149455290092672 &85.846768 & 9.092230 & 7322.1 &-3030.9&0.4$\pm$0.2 & 140$\pm$6 & 398$_{-37}^{46}$ & 1.522$\pm$0.163 & -1.206$\pm$0.134 & 6.156 & 13.395$\pm$0.019 & 13.632$\pm$0.051 & 11.913$\pm$0.040\\
			11 &3336149489649827840 &85.853067 & 9.102319 & 7344.3 &-2994.6&0.4$\pm$0.2 & 155$\pm$9 & 413$_{-8}^{8}$ & 0.809$\pm$0.043 & -2.220$\pm$0.034 & 2.772 & 12.770$\pm$0.003 & 13.482$\pm$0.005 & 11.947$\pm$0.005\\		
			12 &3336109116957457792 &86.037486 & 9.154068 & 7998.5 &-2808.3&1.3$\pm$0.4 & 176$\pm$11 & 396$_{-3}^{3}$ & 1.814$\pm$0.028 & -2.168$\pm$0.016 & 1.574 & 13.299$\pm$0.023 & 14.117$\pm$0.082 & 12.422$\pm$0.058\\
			13 &3336109288756140416 &86.072310 & 9.183034 & 8121.8 &-2704.0&0.8$\pm$0.2 & 137$\pm$4 & 541$_{-22}^{17}$ & 2.018$\pm$0.080 & -3.841$\pm$0.050 & 3.196 & 13.621$\pm$0.007 & 14.320$\pm$0.023 & 12.466$\pm$0.013\\		
			14 &3336111002446797184 &86.080096 & 9.209678 & 8149.1 &-2608.1&0.7$\pm$0.2 & 175$\pm$10 & 374$_{-6}^{6}$ & 1.937$\pm$0.043 & -2.107$\pm$0.027 & 2.285 & 14.006$\pm$0.005 & 15.147$\pm$0.018 & 12.932$\pm$0.011\\
			15 &3336110727568247552 &86.096725 & 9.201062 & 8208.2 &-2639.1&4.1$\pm$0.1 & 18$\pm$6 & 392$_{-3}^{2}$ &  2.980$\pm$0.024 & -2.365$\pm$0.015 & 1.453 & 11.757$\pm$0.003 & 12.315$\pm$0.005 &11.034$\pm$0.005\\
			16 &3336253530937700736 &86.186075 & 9.388527 & 8523.1 &-1964.2&0.6$\pm$0.2 & 164$\pm$8 & 327$_{-23}^{25}$ & 0.222$\pm$0.140 & 1.252$\pm$0.130 & 3.682 & 14.426$\pm$0.013 & 14.899$\pm$0.035 & 12.969$\pm$0.022\\			
			17 &3336093826873858304 &86.339785 & 9.095995 & 9072.5 &-3017.4&1.3$\pm$0.4 & 111$\pm$6 & 368$_{-8}^{9}$ &  1.306$\pm$0.068 & -2.723$\pm$0.044 & 1.932 & 15.336$\pm$0.003 &  16.926$\pm$0.006 & 14.093$\pm$0.005\\
			\hline
		\end{tabular}\\
		{\footnotesize $^{*}$ RA and Dec of the sources are in J2016 epoch obtained from \textit{Gaia} EDR3. $^{\dagger}$ Angular distance of the sources in RA and Dec from $\lambda$ Ori. $^{\ddagger}$ $G$, $G_\mathrm{BP}$, and $G_\mathrm{RP}$ magnitudes obtained from \textit{Gaia} EDR3, presented upto 3 decimal places.}
\end{table}

